A construction of the hat tilings by a Markov partition

We present a simple construction of hat tilings. The construction can be carried out by superimposing a triangular grid on a specially colored image and reading off the orientation of the tiles. We show that our construction produces valid hat tilings, and conversely, in an appropriate sense that is made precise in the paper, that every valid hat tiling can be obtained in this way.

==> SAGEOUTPUTS/fractal_path_depth1_big.tex <==
\def\thefractalbigI
{
(0.0,0.0) -- (0.5,0.866025) -- (1.5,0.866025) -- (1.61803,0.0) -- (2.61803,0.0)
}


==> SAGEOUTPUTS/fractal_path_depth1_big_B.tex <==
\def\thefractalbigBI
{
(0.500000,0.866025) -- (1.500000,0.866025) -- (1.618034,0.000000) -- (2.618034,0.000000)
}


==> SAGEOUTPUTS/fractal_path_depth2_big.tex <==
\def\thefractalbigII
{
(0.0,0.0) -- (0.190983,0.330792) -- (0.5,0.204441) -- (0.690983,0.535233) -- (0.5,0.866025) -- (0.881966,0.866025) -- (0.927051,0.535233) -- (1.30902,0.535233) -- (1.5,0.866025) -- (1.69098,0.535233) -- (1.42705,0.330792) -- (1.61803,0.0) -- (1.80902,0.330792) -- (2.19098,0.330792) -- (2.23607,0.0) -- (2.61803,0.0)
}


==> SAGEOUTPUTS/fractal_path_depth2_big_B.tex <==
\def\thefractalbigBII
{
(0.500000,0.866025) -- (0.881966,0.866025) -- (0.927051,0.535233) -- (1.309017,0.535233) -- (1.500000,0.866025) -- (1.690983,0.535233) -- (1.427051,0.330792) -- (1.618034,0.000000) -- (1.809017,0.330792) -- (2.190983,0.330792) -- (2.236068,0.000000) -- (2.618034,-0.000000)
}


==> SAGEOUTPUTS/fractal_path_depth3_big.tex <==
\def\thefractalbigIII
{
(0.0,0.0) -- (0.072949,0.126351) -- (0.190983,0.0780895) -- (0.263932,0.204441) -- (0.190983,0.330792) -- (0.336881,0.330792) -- (0.354102,0.204441) -- (0.5,0.204441) -- (0.427051,0.330792) -- (0.5,0.457144) -- (0.618034,0.408882) -- (0.690983,0.535233) -- (0.545085,0.535233) -- (0.472136,0.661585) -- (0.572949,0.739674) -- (0.5,0.866025) -- (0.645898,0.866025) -- (0.663119,0.739674) -- (0.809017,0.739674) -- (0.881966,0.866025) -- (0.954915,0.739674) -- (0.854102,0.661585) -- (0.927051,0.535233) -- (1.0,0.661585) -- (1.1459,0.661585) -- (1.16312,0.535233) -- (1.30902,0.535233) -- (1.23607,0.661585) -- (1.30902,0.787936) -- (1.42705,0.739674) -- (1.5,0.866025) -- (1.57295,0.739674) -- (1.47214,0.661585) -- (1.54508,0.535233) -- (1.69098,0.535233) -- (1.61803,0.408882) -- (1.5,0.457144) -- (1.42705,0.330792) -- (1.57295,0.330792) -- (1.6459,0.204441) -- (1.54508,0.126351) -- (1.61803,0.0) -- (1.69098,0.126351) -- (1.80902,0.0780895) -- (1.88197,0.204441) -- (1.80902,0.330792) -- (1.95492,0.330792) -- (1.97214,0.204441) -- (2.11803,0.204441) -- (2.19098,0.330792) -- (2.26393,0.204441) -- (2.16312,0.126351) -- (2.23607,0.0) -- (2.30902,0.126351) -- (2.45492,0.126351) -- (2.47214,0.0) -- (2.61803,0.0)
}


==> SAGEOUTPUTS/fractal_path_depth3_big_B.tex <==
\def\thefractalbigBIII
{
(0.500000,0.866025) -- (0.645898,0.866025) -- (0.663119,0.739674) -- (0.809017,0.739674) -- (0.881966,0.866025) -- (0.954915,0.739674) -- (0.854102,0.661585) -- (0.927051,0.535233) -- (1.000000,0.661585) -- (1.145898,0.661585) -- (1.163119,0.535233) -- (1.309017,0.535233) -- (1.236068,0.661585) -- (1.309017,0.787936) -- (1.427051,0.739674) -- (1.500000,0.866025) -- (1.572949,0.739674) -- (1.472136,0.661585) -- (1.545085,0.535233) -- (1.690983,0.535233) -- (1.618034,0.408882) -- (1.500000,0.457144) -- (1.427051,0.330792) -- (1.572949,0.330792) -- (1.645898,0.204441) -- (1.545085,0.126351) -- (1.618034,-0.000000) -- (1.690983,0.126351) -- (1.809017,0.078089) -- (1.881966,0.204441) -- (1.809017,0.330792) -- (1.954915,0.330792) -- (1.972136,0.204441) -- (2.118034,0.204441) -- (2.190983,0.330792) -- (2.263932,0.204441) -- (2.163119,0.126351) -- (2.236068,-0.000000) -- (2.309017,0.126351) -- (2.454915,0.126351) -- (2.472136,-0.000000) -- (2.618034,-0.000000)
}


==> SAGEOUTPUTS/fractal_path_depth4_big.tex <==
\def\thefractalbigIV
{
(0.0,0.0) -- (0.027864,0.0482619) -- (0.072949,0.0298275) -- (0.100813,0.0780895) -- (0.072949,0.126351) -- (0.128677,0.126351) -- (0.135255,0.0780895) -- (0.190983,0.0780895) -- (0.163119,0.126351) -- (0.190983,0.174613) -- (0.236068,0.156179) -- (0.263932,0.204441) -- (0.208204,0.204441) -- (0.18034,0.252703) -- (0.218847,0.28253) -- (0.190983,0.330792) -- (0.246711,0.330792) -- (0.253289,0.28253) -- (0.309017,0.28253) -- (0.336881,0.330792) -- (0.364745,0.28253) -- (0.326238,0.252703) -- (0.354102,0.204441) -- (0.381966,0.252703) -- (0.437694,0.252703) -- (0.444272,0.204441) -- (0.5,0.204441) -- (0.472136,0.252703) -- (0.510643,0.28253) -- (0.482779,0.330792) -- (0.427051,0.330792) -- (0.454915,0.379054) -- (0.5,0.36062) -- (0.527864,0.408882) -- (0.5,0.457144) -- (0.555728,0.457144) -- (0.562306,0.408882) -- (0.618034,0.408882) -- (0.59017,0.457144) -- (0.618034,0.505406) -- (0.663119,0.486971) -- (0.690983,0.535233) -- (0.635255,0.535233) -- (0.628677,0.583495) -- (0.572949,0.583495) -- (0.545085,0.535233) -- (0.517221,0.583495) -- (0.555728,0.613323) -- (0.527864,0.661585) -- (0.472136,0.661585) -- (0.5,0.709846) -- (0.545085,0.691412) -- (0.572949,0.739674) -- (0.517221,0.739674) -- (0.489357,0.787936) -- (0.527864,0.817763) -- (0.5,0.866025) -- (0.555728,0.866025) -- (0.562306,0.817763) -- (0.618034,0.817763) -- (0.645898,0.866025) -- (0.673762,0.817763) -- (0.635255,0.787936) -- (0.663119,0.739674) -- (0.690983,0.787936) -- (0.746711,0.787936) -- (0.753289,0.739674) -- (0.809017,0.739674) -- (0.781153,0.787936) -- (0.809017,0.836198) -- (0.854102,0.817763) -- (0.881966,0.866025) -- (0.90983,0.817763) -- (0.871323,0.787936) -- (0.899187,0.739674) -- (0.954915,0.739674) -- (0.927051,0.691412) -- (0.881966,0.709846) -- (0.854102,0.661585) -- (0.90983,0.661585) -- (0.937694,0.613323) -- (0.899187,0.583495) -- (0.927051,0.535233) -- (0.954915,0.583495) -- (1.0,0.565061) -- (1.02786,0.613323) -- (1.0,0.661585) -- (1.05573,0.661585) -- (1.06231,0.613323) -- (1.11803,0.613323) -- (1.1459,0.661585) -- (1.17376,0.613323) -- (1.13525,0.583495) -- (1.16312,0.535233) -- (1.19098,0.583495) -- (1.24671,0.583495) -- (1.25329,0.535233) -- (1.30902,0.535233) -- (1.28115,0.583495) -- (1.31966,0.613323) -- (1.2918,0.661585) -- (1.23607,0.661585) -- (1.26393,0.709846) -- (1.30902,0.691412) -- (1.33688,0.739674) -- (1.30902,0.787936) -- (1.36475,0.787936) -- (1.37132,0.739674) -- (1.42705,0.739674) -- (1.39919,0.787936) -- (1.42705,0.836198) -- (1.47214,0.817763) -- (1.5,0.866025) -- (1.52786,0.817763) -- (1.48936,0.787936) -- (1.51722,0.739674) -- (1.57295,0.739674) -- (1.54508,0.691412) -- (1.5,0.709846) -- (1.47214,0.661585) -- (1.52786,0.661585) -- (1.55573,0.613323) -- (1.51722,0.583495) -- (1.54508,0.535233) -- (1.57295,0.583495) -- (1.62868,0.583495) -- (1.63525,0.535233) -- (1.69098,0.535233) -- (1.66312,0.486971) -- (1.61803,0.505406) -- (1.59017,0.457144) -- (1.61803,0.408882) -- (1.56231,0.408882) -- (1.55573,0.457144) -- (1.5,0.457144) -- (1.52786,0.408882) -- (1.5,0.36062) -- (1.45492,0.379054) -- (1.42705,0.330792) -- (1.48278,0.330792) -- (1.48936,0.28253) -- (1.54508,0.28253) -- (1.57295,0.330792) -- (1.60081,0.28253) -- (1.56231,0.252703) -- (1.59017,0.204441) -- (1.6459,0.204441) -- (1.61803,0.156179) -- (1.57295,0.174613) -- (1.54508,0.126351) -- (1.60081,0.126351) -- (1.62868,0.0780895) -- (1.59017,0.0482619) -- (1.61803,0.0) -- (1.6459,0.0482619) -- (1.69098,0.0298275) -- (1.71885,0.0780895) -- (1.69098,0.126351) -- (1.74671,0.126351) -- (1.75329,0.0780895) -- (1.80902,0.0780895) -- (1.78115,0.126351) -- (1.80902,0.174613) -- (1.8541,0.156179) -- (1.88197,0.204441) -- (1.82624,0.204441) -- (1.79837,0.252703) -- (1.83688,0.28253) -- (1.80902,0.330792) -- (1.86475,0.330792) -- (1.87132,0.28253) -- (1.92705,0.28253) -- (1.95492,0.330792) -- (1.98278,0.28253) -- (1.94427,0.252703) -- (1.97214,0.204441) -- (2.0,0.252703) -- (2.05573,0.252703) -- (2.06231,0.204441) -- (2.11803,0.204441) -- (2.09017,0.252703) -- (2.11803,0.300965) -- (2.16312,0.28253) -- (2.19098,0.330792) -- (2.21885,0.28253) -- (2.18034,0.252703) -- (2.2082,0.204441) -- (2.26393,0.204441) -- (2.23607,0.156179) -- (2.19098,0.174613) -- (2.16312,0.126351) -- (2.21885,0.126351) -- (2.24671,0.0780895) -- (2.2082,0.0482619) -- (2.23607,0.0) -- (2.26393,0.0482619) -- (2.30902,0.0298275) -- (2.33688,0.0780895) -- (2.30902,0.126351) -- (2.36475,0.126351) -- (2.37132,0.0780895) -- (2.42705,0.0780895) -- (2.45492,0.126351) -- (2.48278,0.0780895) -- (2.44427,0.0482619) -- (2.47214,0.0) -- (2.5,0.0482619) -- (2.55573,0.0482619) -- (2.56231,0.0) -- (2.61803,0.0)
}


==> SAGEOUTPUTS/fractal_path_depth4_big_B.tex <==
\def\thefractalbigBIV
{
(0.500000,0.866025) -- (0.555728,0.866025) -- (0.562306,0.817763) -- (0.618034,0.817763) -- (0.645898,0.866025) -- (0.673762,0.817763) -- (0.635255,0.787936) -- (0.663119,0.739674) -- (0.690983,0.787936) -- (0.746711,0.787936) -- (0.753289,0.739674) -- (0.809017,0.739674) -- (0.781153,0.787936) -- (0.809017,0.836198) -- (0.854102,0.817763) -- (0.881966,0.866025) -- (0.909830,0.817763) -- (0.871323,0.787936) -- (0.899187,0.739674) -- (0.954915,0.739674) -- (0.927051,0.691412) -- (0.881966,0.709846) -- (0.854102,0.661585) -- (0.909830,0.661585) -- (0.937694,0.613323) -- (0.899187,0.583495) -- (0.927051,0.535233) -- (0.954915,0.583495) -- (1.000000,0.565061) -- (1.027864,0.613323) -- (1.000000,0.661585) -- (1.055728,0.661585) -- (1.062306,0.613323) -- (1.118034,0.613323) -- (1.145898,0.661585) -- (1.173762,0.613323) -- (1.135255,0.583495) -- (1.163119,0.535233) -- (1.190983,0.583495) -- (1.246711,0.583495) -- (1.253289,0.535233) -- (1.309017,0.535233) -- (1.281153,0.583495) -- (1.319660,0.613323) -- (1.291796,0.661585) -- (1.236068,0.661585) -- (1.263932,0.709846) -- (1.309017,0.691412) -- (1.336881,0.739674) -- (1.309017,0.787936) -- (1.364745,0.787936) -- (1.371323,0.739674) -- (1.427051,0.739674) -- (1.399187,0.787936) -- (1.427051,0.836198) -- (1.472136,0.817763) -- (1.500000,0.866025) -- (1.527864,0.817763) -- (1.489357,0.787936) -- (1.517221,0.739674) -- (1.572949,0.739674) -- (1.545085,0.691412) -- (1.500000,0.709846) -- (1.472136,0.661585) -- (1.527864,0.661585) -- (1.555728,0.613323) -- (1.517221,0.583495) -- (1.545085,0.535233) -- (1.572949,0.583495) -- (1.628677,0.583495) -- (1.635255,0.535233) -- (1.690983,0.535233) -- (1.663119,0.486971) -- (1.618034,0.505406) -- (1.590170,0.457144) -- (1.618034,0.408882) -- (1.562306,0.408882) -- (1.555728,0.457144) -- (1.500000,0.457144) -- (1.527864,0.408882) -- (1.500000,0.360620) -- (1.454915,0.379054) -- (1.427051,0.330792) -- (1.482779,0.330792) -- (1.489357,0.282530) -- (1.545085,0.282530) -- (1.572949,0.330792) -- (1.600813,0.282530) -- (1.562306,0.252703) -- (1.590170,0.204441) -- (1.645898,0.204441) -- (1.618034,0.156179) -- (1.572949,0.174613) -- (1.545085,0.126351) -- (1.600813,0.126351) -- (1.628677,0.078089) -- (1.590170,0.048262) -- (1.618034,-0.000000) -- (1.645898,0.048262) -- (1.690983,0.029828) -- (1.718847,0.078089) -- (1.690983,0.126351) -- (1.746711,0.126351) -- (1.753289,0.078089) -- (1.809017,0.078089) -- (1.781153,0.126351) -- (1.809017,0.174613) -- (1.854102,0.156179) -- (1.881966,0.204441) -- (1.826238,0.204441) -- (1.798374,0.252703) -- (1.836881,0.282530) -- (1.809017,0.330792) -- (1.864745,0.330792) -- (1.871323,0.282530) -- (1.927051,0.282530) -- (1.954915,0.330792) -- (1.982779,0.282530) -- (1.944272,0.252703) -- (1.972136,0.204441) -- (2.000000,0.252703) -- (2.055728,0.252703) -- (2.062306,0.204441) -- (2.118034,0.204441) -- (2.090170,0.252703) -- (2.118034,0.300965) -- (2.163119,0.282530) -- (2.190983,0.330792) -- (2.218847,0.282530) -- (2.180340,0.252703) -- (2.208204,0.204441) -- (2.263932,0.204441) -- (2.236068,0.156179) -- (2.190983,0.174613) -- (2.163119,0.126351) -- (2.218847,0.126351) -- (2.246711,0.078089) -- (2.208204,0.048262) -- (2.236068,-0.000000) -- (2.263932,0.048262) -- (2.309017,0.029828) -- (2.336881,0.078089) -- (2.309017,0.126351) -- (2.364745,0.126351) -- (2.371323,0.078089) -- (2.427051,0.078089) -- (2.454915,0.126351) -- (2.482779,0.078089) -- (2.444272,0.048262) -- (2.472136,-0.000000) -- (2.500000,0.048262) -- (2.555728,0.048262) -- (2.562306,-0.000000) -- (2.618034,-0.000000)
}


==> SAGEOUTPUTS/fractal_path_depth5_big.tex <==
\def\thefractalbigV
{
(0.0,0.0) -- (0.0106431,0.0184344) -- (0.027864,0.0113931) -- (0.0385072,0.0298275) -- (0.027864,0.0482619) -- (0.0491503,0.0482619) -- (0.0516628,0.0298275) -- (0.072949,0.0298275) -- (0.0623059,0.0482619) -- (0.072949,0.0666964) -- (0.0901699,0.059655) -- (0.100813,0.0780895) -- (0.0795268,0.0780895) -- (0.0688837,0.0965239) -- (0.0835921,0.107917) -- (0.072949,0.126351) -- (0.0942353,0.126351) -- (0.0967478,0.107917) -- (0.118034,0.107917) -- (0.128677,0.126351) -- (0.13932,0.107917) -- (0.124612,0.0965239) -- (0.135255,0.0780895) -- (0.145898,0.0965239) -- (0.167184,0.0965239) -- (0.169697,0.0780895) -- (0.190983,0.0780895) -- (0.18034,0.0965239) -- (0.195048,0.107917) -- (0.184405,0.126351) -- (0.163119,0.126351) -- (0.173762,0.144786) -- (0.190983,0.137745) -- (0.201626,0.156179) -- (0.190983,0.174613) -- (0.212269,0.174613) -- (0.214782,0.156179) -- (0.236068,0.156179) -- (0.225425,0.174613) -- (0.236068,0.193048) -- (0.253289,0.186006) -- (0.263932,0.204441) -- (0.242646,0.204441) -- (0.240133,0.222875) -- (0.218847,0.222875) -- (0.208204,0.204441) -- (0.197561,0.222875) -- (0.212269,0.234268) -- (0.201626,0.252703) -- (0.18034,0.252703) -- (0.190983,0.271137) -- (0.208204,0.264096) -- (0.218847,0.28253) -- (0.197561,0.28253) -- (0.186918,0.300965) -- (0.201626,0.312358) -- (0.190983,0.330792) -- (0.212269,0.330792) -- (0.214782,0.312358) -- (0.236068,0.312358) -- (0.246711,0.330792) -- (0.257354,0.312358) -- (0.242646,0.300965) -- (0.253289,0.28253) -- (0.263932,0.300965) -- (0.285218,0.300965) -- (0.287731,0.28253) -- (0.309017,0.28253) -- (0.298374,0.300965) -- (0.309017,0.319399) -- (0.326238,0.312358) -- (0.336881,0.330792) -- (0.347524,0.312358) -- (0.332816,0.300965) -- (0.343459,0.28253) -- (0.364745,0.28253) -- (0.354102,0.264096) -- (0.336881,0.271137) -- (0.326238,0.252703) -- (0.347524,0.252703) -- (0.358167,0.234268) -- (0.343459,0.222875) -- (0.354102,0.204441) -- (0.364745,0.222875) -- (0.381966,0.215834) -- (0.392609,0.234268) -- (0.381966,0.252703) -- (0.403252,0.252703) -- (0.405765,0.234268) -- (0.427051,0.234268) -- (0.437694,0.252703) -- (0.448337,0.234268) -- (0.433629,0.222875) -- (0.444272,0.204441) -- (0.454915,0.222875) -- (0.476201,0.222875) -- (0.478714,0.204441) -- (0.5,0.204441) -- (0.489357,0.222875) -- (0.504065,0.234268) -- (0.493422,0.252703) -- (0.472136,0.252703) -- (0.482779,0.271137) -- (0.5,0.264096) -- (0.510643,0.28253) -- (0.489357,0.28253) -- (0.478714,0.300965) -- (0.493422,0.312358) -- (0.482779,0.330792) -- (0.472136,0.312358) -- (0.45085,0.312358) -- (0.448337,0.330792) -- (0.427051,0.330792) -- (0.437694,0.349227) -- (0.454915,0.342185) -- (0.465558,0.36062) -- (0.454915,0.379054) -- (0.476201,0.379054) -- (0.478714,0.36062) -- (0.5,0.36062) -- (0.489357,0.379054) -- (0.5,0.397489) -- (0.517221,0.390447) -- (0.527864,0.408882) -- (0.506578,0.408882) -- (0.495935,0.427316) -- (0.510643,0.438709) -- (0.5,0.457144) -- (0.521286,0.457144) -- (0.523799,0.438709) -- (0.545085,0.438709) -- (0.555728,0.457144) -- (0.566371,0.438709) -- (0.551663,0.427316) -- (0.562306,0.408882) -- (0.572949,0.427316) -- (0.594235,0.427316) -- (0.596748,0.408882) -- (0.618034,0.408882) -- (0.607391,0.427316) -- (0.622099,0.438709) -- (0.611456,0.457144) -- (0.59017,0.457144) -- (0.600813,0.475578) -- (0.618034,0.468537) -- (0.628677,0.486971) -- (0.618034,0.505406) -- (0.63932,0.505406) -- (0.641833,0.486971) -- (0.663119,0.486971) -- (0.652476,0.505406) -- (0.663119,0.52384) -- (0.68034,0.516799) -- (0.690983,0.535233) -- (0.669697,0.535233) -- (0.667184,0.553668) -- (0.645898,0.553668) -- (0.635255,0.535233) -- (0.624612,0.553668) -- (0.63932,0.565061) -- (0.628677,0.583495) -- (0.618034,0.565061) -- (0.596748,0.565061) -- (0.594235,0.583495) -- (0.572949,0.583495) -- (0.583592,0.565061) -- (0.572949,0.546626) -- (0.555728,0.553668) -- (0.545085,0.535233) -- (0.534442,0.553668) -- (0.54915,0.565061) -- (0.538507,0.583495) -- (0.517221,0.583495) -- (0.527864,0.601929) -- (0.545085,0.594888) -- (0.555728,0.613323) -- (0.534442,0.613323) -- (0.523799,0.631757) -- (0.538507,0.64315) -- (0.527864,0.661585) -- (0.517221,0.64315) -- (0.495935,0.64315) -- (0.493422,0.661585) -- (0.472136,0.661585) -- (0.482779,0.680019) -- (0.5,0.672978) -- (0.510643,0.691412) -- (0.5,0.709846) -- (0.521286,0.709846) -- (0.523799,0.691412) -- (0.545085,0.691412) -- (0.534442,0.709846) -- (0.545085,0.728281) -- (0.562306,0.72124) -- (0.572949,0.739674) -- (0.551663,0.739674) -- (0.54915,0.758108) -- (0.527864,0.758108) -- (0.517221,0.739674) -- (0.506578,0.758108) -- (0.521286,0.769502) -- (0.510643,0.787936) -- (0.489357,0.787936) -- (0.5,0.80637) -- (0.517221,0.799329) -- (0.527864,0.817763) -- (0.506578,0.817763) -- (0.495935,0.836198) -- (0.510643,0.847591) -- (0.5,0.866025) -- (0.521286,0.866025) -- (0.523799,0.847591) -- (0.545085,0.847591) -- (0.555728,0.866025) -- (0.566371,0.847591) -- (0.551663,0.836198) -- (0.562306,0.817763) -- (0.572949,0.836198) -- (0.594235,0.836198) -- (0.596748,0.817763) -- (0.618034,0.817763) -- (0.607391,0.836198) -- (0.618034,0.854632) -- (0.635255,0.847591) -- (0.645898,0.866025) -- (0.656541,0.847591) -- (0.641833,0.836198) -- (0.652476,0.817763) -- (0.673762,0.817763) -- (0.663119,0.799329) -- (0.645898,0.80637) -- (0.635255,0.787936) -- (0.656541,0.787936) -- (0.667184,0.769502) -- (0.652476,0.758108) -- (0.663119,0.739674) -- (0.673762,0.758108) -- (0.690983,0.751067) -- (0.701626,0.769502) -- (0.690983,0.787936) -- (0.712269,0.787936) -- (0.714782,0.769502) -- (0.736068,0.769502) -- (0.746711,0.787936) -- (0.757354,0.769502) -- (0.742646,0.758108) -- (0.753289,0.739674) -- (0.763932,0.758108) -- (0.785218,0.758108) -- (0.787731,0.739674) -- (0.809017,0.739674) -- (0.798374,0.758108) -- (0.813082,0.769502) -- (0.802439,0.787936) -- (0.781153,0.787936) -- (0.791796,0.80637) -- (0.809017,0.799329) -- (0.81966,0.817763) -- (0.809017,0.836198) -- (0.830303,0.836198) -- (0.832816,0.817763) -- (0.854102,0.817763) -- (0.843459,0.836198) -- (0.854102,0.854632) -- (0.871323,0.847591) -- (0.881966,0.866025) -- (0.892609,0.847591) -- (0.877901,0.836198) -- (0.888544,0.817763) -- (0.90983,0.817763) -- (0.899187,0.799329) -- (0.881966,0.80637) -- (0.871323,0.787936) -- (0.892609,0.787936) -- (0.903252,0.769502) -- (0.888544,0.758108) -- (0.899187,0.739674) -- (0.90983,0.758108) -- (0.931116,0.758108) -- (0.933629,0.739674) -- (0.954915,0.739674) -- (0.944272,0.72124) -- (0.927051,0.728281) -- (0.916408,0.709846) -- (0.927051,0.691412) -- (0.905765,0.691412) -- (0.903252,0.709846) -- (0.881966,0.709846) -- (0.892609,0.691412) -- (0.881966,0.672978) -- (0.864745,0.680019) -- (0.854102,0.661585) -- (0.875388,0.661585) -- (0.877901,0.64315) -- (0.899187,0.64315) -- (0.90983,0.661585) -- (0.920473,0.64315) -- (0.905765,0.631757) -- (0.916408,0.613323) -- (0.937694,0.613323) -- (0.927051,0.594888) -- (0.90983,0.601929) -- (0.899187,0.583495) -- (0.920473,0.583495) -- (0.931116,0.565061) -- (0.916408,0.553668) -- (0.927051,0.535233) -- (0.937694,0.553668) -- (0.954915,0.546626) -- (0.965558,0.565061) -- (0.954915,0.583495) -- (0.976201,0.583495) -- (0.978714,0.565061) -- (1.0,0.565061) -- (0.989357,0.583495) -- (1.0,0.601929) -- (1.01722,0.594888) -- (1.02786,0.613323) -- (1.00658,0.613323) -- (0.995935,0.631757) -- (1.01064,0.64315) -- (1.0,0.661585) -- (1.02129,0.661585) -- (1.0238,0.64315) -- (1.04508,0.64315) -- (1.05573,0.661585) -- (1.06637,0.64315) -- (1.05166,0.631757) -- (1.06231,0.613323) -- (1.07295,0.631757) -- (1.09424,0.631757) -- (1.09675,0.613323) -- (1.11803,0.613323) -- (1.10739,0.631757) -- (1.11803,0.650191) -- (1.13525,0.64315) -- (1.1459,0.661585) -- (1.15654,0.64315) -- (1.14183,0.631757) -- (1.15248,0.613323) -- (1.17376,0.613323) -- (1.16312,0.594888) -- (1.1459,0.601929) -- (1.13525,0.583495) -- (1.15654,0.583495) -- (1.16718,0.565061) -- (1.15248,0.553668) -- (1.16312,0.535233) -- (1.17376,0.553668) -- (1.19098,0.546626) -- (1.20163,0.565061) -- (1.19098,0.583495) -- (1.21227,0.583495) -- (1.21478,0.565061) -- (1.23607,0.565061) -- (1.24671,0.583495) -- (1.25735,0.565061) -- (1.24265,0.553668) -- (1.25329,0.535233) -- (1.26393,0.553668) -- (1.28522,0.553668) -- (1.28773,0.535233) -- (1.30902,0.535233) -- (1.29837,0.553668) -- (1.31308,0.565061) -- (1.30244,0.583495) -- (1.28115,0.583495) -- (1.2918,0.601929) -- (1.30902,0.594888) -- (1.31966,0.613323) -- (1.29837,0.613323) -- (1.28773,0.631757) -- (1.30244,0.64315) -- (1.2918,0.661585) -- (1.28115,0.64315) -- (1.25987,0.64315) -- (1.25735,0.661585) -- (1.23607,0.661585) -- (1.24671,0.680019) -- (1.26393,0.672978) -- (1.27458,0.691412) -- (1.26393,0.709846) -- (1.28522,0.709846) -- (1.28773,0.691412) -- (1.30902,0.691412) -- (1.29837,0.709846) -- (1.30902,0.728281) -- (1.32624,0.72124) -- (1.33688,0.739674) -- (1.31559,0.739674) -- (1.30495,0.758108) -- (1.31966,0.769502) -- (1.30902,0.787936) -- (1.3303,0.787936) -- (1.33282,0.769502) -- (1.3541,0.769502) -- (1.36475,0.787936) -- (1.37539,0.769502) -- (1.36068,0.758108) -- (1.37132,0.739674) -- (1.38197,0.758108) -- (1.40325,0.758108) -- (1.40576,0.739674) -- (1.42705,0.739674) -- (1.41641,0.758108) -- (1.43112,0.769502) -- (1.42047,0.787936) -- (1.39919,0.787936) -- (1.40983,0.80637) -- (1.42705,0.799329) -- (1.43769,0.817763) -- (1.42705,0.836198) -- (1.44834,0.836198) -- (1.45085,0.817763) -- (1.47214,0.817763) -- (1.46149,0.836198) -- (1.47214,0.854632) -- (1.48936,0.847591) -- (1.5,0.866025) -- (1.51064,0.847591) -- (1.49593,0.836198) -- (1.50658,0.817763) -- (1.52786,0.817763) -- (1.51722,0.799329) -- (1.5,0.80637) -- (1.48936,0.787936) -- (1.51064,0.787936) -- (1.52129,0.769502) -- (1.50658,0.758108) -- (1.51722,0.739674) -- (1.52786,0.758108) -- (1.54915,0.758108) -- (1.55166,0.739674) -- (1.57295,0.739674) -- (1.56231,0.72124) -- (1.54508,0.728281) -- (1.53444,0.709846) -- (1.54508,0.691412) -- (1.5238,0.691412) -- (1.52129,0.709846) -- (1.5,0.709846) -- (1.51064,0.691412) -- (1.5,0.672978) -- (1.48278,0.680019) -- (1.47214,0.661585) -- (1.49342,0.661585) -- (1.49593,0.64315) -- (1.51722,0.64315) -- (1.52786,0.661585) -- (1.53851,0.64315) -- (1.5238,0.631757) -- (1.53444,0.613323) -- (1.55573,0.613323) -- (1.54508,0.594888) -- (1.52786,0.601929) -- (1.51722,0.583495) -- (1.53851,0.583495) -- (1.54915,0.565061) -- (1.53444,0.553668) -- (1.54508,0.535233) -- (1.55573,0.553668) -- (1.57295,0.546626) -- (1.58359,0.565061) -- (1.57295,0.583495) -- (1.59424,0.583495) -- (1.59675,0.565061) -- (1.61803,0.565061) -- (1.62868,0.583495) -- (1.63932,0.565061) -- (1.62461,0.553668) -- (1.63525,0.535233) -- (1.6459,0.553668) -- (1.66718,0.553668) -- (1.6697,0.535233) -- (1.69098,0.535233) -- (1.68034,0.516799) -- (1.66312,0.52384) -- (1.65248,0.505406) -- (1.66312,0.486971) -- (1.64183,0.486971) -- (1.63932,0.505406) -- (1.61803,0.505406) -- (1.62868,0.486971) -- (1.61803,0.468537) -- (1.60081,0.475578) -- (1.59017,0.457144) -- (1.61146,0.457144) -- (1.6221,0.438709) -- (1.60739,0.427316) -- (1.61803,0.408882) -- (1.59675,0.408882) -- (1.59424,0.427316) -- (1.57295,0.427316) -- (1.56231,0.408882) -- (1.55166,0.427316) -- (1.56637,0.438709) -- (1.55573,0.457144) -- (1.54508,0.438709) -- (1.5238,0.438709) -- (1.52129,0.457144) -- (1.5,0.457144) -- (1.51064,0.438709) -- (1.49593,0.427316) -- (1.50658,0.408882) -- (1.52786,0.408882) -- (1.51722,0.390447) -- (1.5,0.397489) -- (1.48936,0.379054) -- (1.5,0.36062) -- (1.47871,0.36062) -- (1.4762,0.379054) -- (1.45492,0.379054) -- (1.46556,0.36062) -- (1.45492,0.342185) -- (1.43769,0.349227) -- (1.42705,0.330792) -- (1.44834,0.330792) -- (1.45085,0.312358) -- (1.47214,0.312358) -- (1.48278,0.330792) -- (1.49342,0.312358) -- (1.47871,0.300965) -- (1.48936,0.28253) -- (1.5,0.300965) -- (1.52129,0.300965) -- (1.5238,0.28253) -- (1.54508,0.28253) -- (1.53444,0.300965) -- (1.54508,0.319399) -- (1.56231,0.312358) -- (1.57295,0.330792) -- (1.58359,0.312358) -- (1.56888,0.300965) -- (1.57953,0.28253) -- (1.60081,0.28253) -- (1.59017,0.264096) -- (1.57295,0.271137) -- (1.56231,0.252703) -- (1.58359,0.252703) -- (1.59424,0.234268) -- (1.57953,0.222875) -- (1.59017,0.204441) -- (1.60081,0.222875) -- (1.6221,0.222875) -- (1.62461,0.204441) -- (1.6459,0.204441) -- (1.63525,0.186006) -- (1.61803,0.193048) -- (1.60739,0.174613) -- (1.61803,0.156179) -- (1.59675,0.156179) -- (1.59424,0.174613) -- (1.57295,0.174613) -- (1.58359,0.156179) -- (1.57295,0.137745) -- (1.55573,0.144786) -- (1.54508,0.126351) -- (1.56637,0.126351) -- (1.56888,0.107917) -- (1.59017,0.107917) -- (1.60081,0.126351) -- (1.61146,0.107917) -- (1.59675,0.0965239) -- (1.60739,0.0780895) -- (1.62868,0.0780895) -- (1.61803,0.059655) -- (1.60081,0.0666964) -- (1.59017,0.0482619) -- (1.61146,0.0482619) -- (1.6221,0.0298275) -- (1.60739,0.0184344) -- (1.61803,0.0) -- (1.62868,0.0184344) -- (1.6459,0.0113931) -- (1.65654,0.0298275) -- (1.6459,0.0482619) -- (1.66718,0.0482619) -- (1.6697,0.0298275) -- (1.69098,0.0298275) -- (1.68034,0.0482619) -- (1.69098,0.0666964) -- (1.7082,0.059655) -- (1.71885,0.0780895) -- (1.69756,0.0780895) -- (1.68692,0.0965239) -- (1.70163,0.107917) -- (1.69098,0.126351) -- (1.71227,0.126351) -- (1.71478,0.107917) -- (1.73607,0.107917) -- (1.74671,0.126351) -- (1.75735,0.107917) -- (1.74265,0.0965239) -- (1.75329,0.0780895) -- (1.76393,0.0965239) -- (1.78522,0.0965239) -- (1.78773,0.0780895) -- (1.80902,0.0780895) -- (1.79837,0.0965239) -- (1.81308,0.107917) -- (1.80244,0.126351) -- (1.78115,0.126351) -- (1.7918,0.144786) -- (1.80902,0.137745) -- (1.81966,0.156179) -- (1.80902,0.174613) -- (1.8303,0.174613) -- (1.83282,0.156179) -- (1.8541,0.156179) -- (1.84346,0.174613) -- (1.8541,0.193048) -- (1.87132,0.186006) -- (1.88197,0.204441) -- (1.86068,0.204441) -- (1.85817,0.222875) -- (1.83688,0.222875) -- (1.82624,0.204441) -- (1.81559,0.222875) -- (1.8303,0.234268) -- (1.81966,0.252703) -- (1.79837,0.252703) -- (1.80902,0.271137) -- (1.82624,0.264096) -- (1.83688,0.28253) -- (1.81559,0.28253) -- (1.80495,0.300965) -- (1.81966,0.312358) -- (1.80902,0.330792) -- (1.8303,0.330792) -- (1.83282,0.312358) -- (1.8541,0.312358) -- (1.86475,0.330792) -- (1.87539,0.312358) -- (1.86068,0.300965) -- (1.87132,0.28253) -- (1.88197,0.300965) -- (1.90325,0.300965) -- (1.90576,0.28253) -- (1.92705,0.28253) -- (1.91641,0.300965) -- (1.92705,0.319399) -- (1.94427,0.312358) -- (1.95492,0.330792) -- (1.96556,0.312358) -- (1.95085,0.300965) -- (1.96149,0.28253) -- (1.98278,0.28253) -- (1.97214,0.264096) -- (1.95492,0.271137) -- (1.94427,0.252703) -- (1.96556,0.252703) -- (1.9762,0.234268) -- (1.96149,0.222875) -- (1.97214,0.204441) -- (1.98278,0.222875) -- (2.0,0.215834) -- (2.01064,0.234268) -- (2.0,0.252703) -- (2.02129,0.252703) -- (2.0238,0.234268) -- (2.04508,0.234268) -- (2.05573,0.252703) -- (2.06637,0.234268) -- (2.05166,0.222875) -- (2.06231,0.204441) -- (2.07295,0.222875) -- (2.09424,0.222875) -- (2.09675,0.204441) -- (2.11803,0.204441) -- (2.10739,0.222875) -- (2.1221,0.234268) -- (2.11146,0.252703) -- (2.09017,0.252703) -- (2.10081,0.271137) -- (2.11803,0.264096) -- (2.12868,0.28253) -- (2.11803,0.300965) -- (2.13932,0.300965) -- (2.14183,0.28253) -- (2.16312,0.28253) -- (2.15248,0.300965) -- (2.16312,0.319399) -- (2.18034,0.312358) -- (2.19098,0.330792) -- (2.20163,0.312358) -- (2.18692,0.300965) -- (2.19756,0.28253) -- (2.21885,0.28253) -- (2.2082,0.264096) -- (2.19098,0.271137) -- (2.18034,0.252703) -- (2.20163,0.252703) -- (2.21227,0.234268) -- (2.19756,0.222875) -- (2.2082,0.204441) -- (2.21885,0.222875) -- (2.24013,0.222875) -- (2.24265,0.204441) -- (2.26393,0.204441) -- (2.25329,0.186006) -- (2.23607,0.193048) -- (2.22542,0.174613) -- (2.23607,0.156179) -- (2.21478,0.156179) -- (2.21227,0.174613) -- (2.19098,0.174613) -- (2.20163,0.156179) -- (2.19098,0.137745) -- (2.17376,0.144786) -- (2.16312,0.126351) -- (2.18441,0.126351) -- (2.18692,0.107917) -- (2.2082,0.107917) -- (2.21885,0.126351) -- (2.22949,0.107917) -- (2.21478,0.0965239) -- (2.22542,0.0780895) -- (2.24671,0.0780895) -- (2.23607,0.059655) -- (2.21885,0.0666964) -- (2.2082,0.0482619) -- (2.22949,0.0482619) -- (2.24013,0.0298275) -- (2.22542,0.0184344) -- (2.23607,0.0) -- (2.24671,0.0184344) -- (2.26393,0.0113931) -- (2.27458,0.0298275) -- (2.26393,0.0482619) -- (2.28522,0.0482619) -- (2.28773,0.0298275) -- (2.30902,0.0298275) -- (2.29837,0.0482619) -- (2.30902,0.0666964) -- (2.32624,0.059655) -- (2.33688,0.0780895) -- (2.31559,0.0780895) -- (2.30495,0.0965239) -- (2.31966,0.107917) -- (2.30902,0.126351) -- (2.3303,0.126351) -- (2.33282,0.107917) -- (2.3541,0.107917) -- (2.36475,0.126351) -- (2.37539,0.107917) -- (2.36068,0.0965239) -- (2.37132,0.0780895) -- (2.38197,0.0965239) -- (2.40325,0.0965239) -- (2.40576,0.0780895) -- (2.42705,0.0780895) -- (2.41641,0.0965239) -- (2.42705,0.114958) -- (2.44427,0.107917) -- (2.45492,0.126351) -- (2.46556,0.107917) -- (2.45085,0.0965239) -- (2.46149,0.0780895) -- (2.48278,0.0780895) -- (2.47214,0.059655) -- (2.45492,0.0666964) -- (2.44427,0.0482619) -- (2.46556,0.0482619) -- (2.4762,0.0298275) -- (2.46149,0.0184344) -- (2.47214,0.0) -- (2.48278,0.0184344) -- (2.5,0.0113931) -- (2.51064,0.0298275) -- (2.5,0.0482619) -- (2.52129,0.0482619) -- (2.5238,0.0298275) -- (2.54508,0.0298275) -- (2.55573,0.0482619) -- (2.56637,0.0298275) -- (2.55166,0.0184344) -- (2.56231,0.0) -- (2.57295,0.0184344) -- (2.59424,0.0184344) -- (2.59675,0.0) -- (2.61803,0.0)
}


==> SAGEOUTPUTS/fractal_path_depth5_big_B.tex <==
\def\thefractalbigBV
{
(0.500000,0.866025) -- (0.521286,0.866025) -- (0.523799,0.847591) -- (0.545085,0.847591) -- (0.555728,0.866025) -- (0.566371,0.847591) -- (0.551663,0.836198) -- (0.562306,0.817763) -- (0.572949,0.836198) -- (0.594235,0.836198) -- (0.596748,0.817763) -- (0.618034,0.817763) -- (0.607391,0.836198) -- (0.618034,0.854632) -- (0.635255,0.847591) -- (0.645898,0.866025) -- (0.656541,0.847591) -- (0.641833,0.836198) -- (0.652476,0.817763) -- (0.673762,0.817763) -- (0.663119,0.799329) -- (0.645898,0.806370) -- (0.635255,0.787936) -- (0.656541,0.787936) -- (0.667184,0.769502) -- (0.652476,0.758108) -- (0.663119,0.739674) -- (0.673762,0.758108) -- (0.690983,0.751067) -- (0.701626,0.769502) -- (0.690983,0.787936) -- (0.712269,0.787936) -- (0.714782,0.769502) -- (0.736068,0.769502) -- (0.746711,0.787936) -- (0.757354,0.769502) -- (0.742646,0.758108) -- (0.753289,0.739674) -- (0.763932,0.758108) -- (0.785218,0.758108) -- (0.787731,0.739674) -- (0.809017,0.739674) -- (0.798374,0.758108) -- (0.813082,0.769502) -- (0.802439,0.787936) -- (0.781153,0.787936) -- (0.791796,0.806370) -- (0.809017,0.799329) -- (0.819660,0.817763) -- (0.809017,0.836198) -- (0.830303,0.836198) -- (0.832816,0.817763) -- (0.854102,0.817763) -- (0.843459,0.836198) -- (0.854102,0.854632) -- (0.871323,0.847591) -- (0.881966,0.866025) -- (0.892609,0.847591) -- (0.877901,0.836198) -- (0.888544,0.817763) -- (0.909830,0.817763) -- (0.899187,0.799329) -- (0.881966,0.806370) -- (0.871323,0.787936) -- (0.892609,0.787936) -- (0.903252,0.769502) -- (0.888544,0.758108) -- (0.899187,0.739674) -- (0.909830,0.758108) -- (0.931116,0.758108) -- (0.933629,0.739674) -- (0.954915,0.739674) -- (0.944272,0.721240) -- (0.927051,0.728281) -- (0.916408,0.709846) -- (0.927051,0.691412) -- (0.905765,0.691412) -- (0.903252,0.709846) -- (0.881966,0.709846) -- (0.892609,0.691412) -- (0.881966,0.672978) -- (0.864745,0.680019) -- (0.854102,0.661585) -- (0.875388,0.661585) -- (0.877901,0.643150) -- (0.899187,0.643150) -- (0.909830,0.661585) -- (0.920473,0.643150) -- (0.905765,0.631757) -- (0.916408,0.613323) -- (0.937694,0.613323) -- (0.927051,0.594888) -- (0.909830,0.601929) -- (0.899187,0.583495) -- (0.920473,0.583495) -- (0.931116,0.565061) -- (0.916408,0.553668) -- (0.927051,0.535233) -- (0.937694,0.553668) -- (0.954915,0.546626) -- (0.965558,0.565061) -- (0.954915,0.583495) -- (0.976201,0.583495) -- (0.978714,0.565061) -- (1.000000,0.565061) -- (0.989357,0.583495) -- (1.000000,0.601929) -- (1.017221,0.594888) -- (1.027864,0.613323) -- (1.006578,0.613323) -- (0.995935,0.631757) -- (1.010643,0.643150) -- (1.000000,0.661585) -- (1.021286,0.661585) -- (1.023799,0.643150) -- (1.045085,0.643150) -- (1.055728,0.661585) -- (1.066371,0.643150) -- (1.051663,0.631757) -- (1.062306,0.613323) -- (1.072949,0.631757) -- (1.094235,0.631757) -- (1.096748,0.613323) -- (1.118034,0.613323) -- (1.107391,0.631757) -- (1.118034,0.650191) -- (1.135255,0.643150) -- (1.145898,0.661585) -- (1.156541,0.643150) -- (1.141833,0.631757) -- (1.152476,0.613323) -- (1.173762,0.613323) -- (1.163119,0.594888) -- (1.145898,0.601929) -- (1.135255,0.583495) -- (1.156541,0.583495) -- (1.167184,0.565061) -- (1.152476,0.553668) -- (1.163119,0.535233) -- (1.173762,0.553668) -- (1.190983,0.546626) -- (1.201626,0.565061) -- (1.190983,0.583495) -- (1.212269,0.583495) -- (1.214782,0.565061) -- (1.236068,0.565061) -- (1.246711,0.583495) -- (1.257354,0.565061) -- (1.242646,0.553668) -- (1.253289,0.535233) -- (1.263932,0.553668) -- (1.285218,0.553668) -- (1.287731,0.535233) -- (1.309017,0.535233) -- (1.298374,0.553668) -- (1.313082,0.565061) -- (1.302439,0.583495) -- (1.281153,0.583495) -- (1.291796,0.601929) -- (1.309017,0.594888) -- (1.319660,0.613323) -- (1.298374,0.613323) -- (1.287731,0.631757) -- (1.302439,0.643150) -- (1.291796,0.661585) -- (1.281153,0.643150) -- (1.259867,0.643150) -- (1.257354,0.661585) -- (1.236068,0.661585) -- (1.246711,0.680019) -- (1.263932,0.672978) -- (1.274575,0.691412) -- (1.263932,0.709846) -- (1.285218,0.709846) -- (1.287731,0.691412) -- (1.309017,0.691412) -- (1.298374,0.709846) -- (1.309017,0.728281) -- (1.326238,0.721240) -- (1.336881,0.739674) -- (1.315595,0.739674) -- (1.304952,0.758108) -- (1.319660,0.769502) -- (1.309017,0.787936) -- (1.330303,0.787936) -- (1.332816,0.769502) -- (1.354102,0.769502) -- (1.364745,0.787936) -- (1.375388,0.769502) -- (1.360680,0.758108) -- (1.371323,0.739674) -- (1.381966,0.758108) -- (1.403252,0.758108) -- (1.405765,0.739674) -- (1.427051,0.739674) -- (1.416408,0.758108) -- (1.431116,0.769502) -- (1.420473,0.787936) -- (1.399187,0.787936) -- (1.409830,0.806370) -- (1.427051,0.799329) -- (1.437694,0.817763) -- (1.427051,0.836198) -- (1.448337,0.836198) -- (1.450850,0.817763) -- (1.472136,0.817763) -- (1.461493,0.836198) -- (1.472136,0.854632) -- (1.489357,0.847591) -- (1.500000,0.866025) -- (1.510643,0.847591) -- (1.495935,0.836198) -- (1.506578,0.817763) -- (1.527864,0.817763) -- (1.517221,0.799329) -- (1.500000,0.806370) -- (1.489357,0.787936) -- (1.510643,0.787936) -- (1.521286,0.769502) -- (1.506578,0.758108) -- (1.517221,0.739674) -- (1.527864,0.758108) -- (1.549150,0.758108) -- (1.551663,0.739674) -- (1.572949,0.739674) -- (1.562306,0.721240) -- (1.545085,0.728281) -- (1.534442,0.709846) -- (1.545085,0.691412) -- (1.523799,0.691412) -- (1.521286,0.709846) -- (1.500000,0.709846) -- (1.510643,0.691412) -- (1.500000,0.672978) -- (1.482779,0.680019) -- (1.472136,0.661585) -- (1.493422,0.661585) -- (1.495935,0.643150) -- (1.517221,0.643150) -- (1.527864,0.661585) -- (1.538507,0.643150) -- (1.523799,0.631757) -- (1.534442,0.613323) -- (1.555728,0.613323) -- (1.545085,0.594888) -- (1.527864,0.601929) -- (1.517221,0.583495) -- (1.538507,0.583495) -- (1.549150,0.565061) -- (1.534442,0.553668) -- (1.545085,0.535233) -- (1.555728,0.553668) -- (1.572949,0.546626) -- (1.583592,0.565061) -- (1.572949,0.583495) -- (1.594235,0.583495) -- (1.596748,0.565061) -- (1.618034,0.565061) -- (1.628677,0.583495) -- (1.639320,0.565061) -- (1.624612,0.553668) -- (1.635255,0.535233) -- (1.645898,0.553668) -- (1.667184,0.553668) -- (1.669697,0.535233) -- (1.690983,0.535233) -- (1.680340,0.516799) -- (1.663119,0.523840) -- (1.652476,0.505406) -- (1.663119,0.486971) -- (1.641833,0.486971) -- (1.639320,0.505406) -- (1.618034,0.505406) -- (1.628677,0.486971) -- (1.618034,0.468537) -- (1.600813,0.475578) -- (1.590170,0.457144) -- (1.611456,0.457144) -- (1.622099,0.438709) -- (1.607391,0.427316) -- (1.618034,0.408882) -- (1.596748,0.408882) -- (1.594235,0.427316) -- (1.572949,0.427316) -- (1.562306,0.408882) -- (1.551663,0.427316) -- (1.566371,0.438709) -- (1.555728,0.457144) -- (1.545085,0.438709) -- (1.523799,0.438709) -- (1.521286,0.457144) -- (1.500000,0.457144) -- (1.510643,0.438709) -- (1.495935,0.427316) -- (1.506578,0.408882) -- (1.527864,0.408882) -- (1.517221,0.390447) -- (1.500000,0.397489) -- (1.489357,0.379054) -- (1.500000,0.360620) -- (1.478714,0.360620) -- (1.476201,0.379054) -- (1.454915,0.379054) -- (1.465558,0.360620) -- (1.454915,0.342185) -- (1.437694,0.349227) -- (1.427051,0.330792) -- (1.448337,0.330792) -- (1.450850,0.312358) -- (1.472136,0.312358) -- (1.482779,0.330792) -- (1.493422,0.312358) -- (1.478714,0.300965) -- (1.489357,0.282530) -- (1.500000,0.300965) -- (1.521286,0.300965) -- (1.523799,0.282530) -- (1.545085,0.282530) -- (1.534442,0.300965) -- (1.545085,0.319399) -- (1.562306,0.312358) -- (1.572949,0.330792) -- (1.583592,0.312358) -- (1.568884,0.300965) -- (1.579527,0.282530) -- (1.600813,0.282530) -- (1.590170,0.264096) -- (1.572949,0.271137) -- (1.562306,0.252703) -- (1.583592,0.252703) -- (1.594235,0.234268) -- (1.579527,0.222875) -- (1.590170,0.204441) -- (1.600813,0.222875) -- (1.622099,0.222875) -- (1.624612,0.204441) -- (1.645898,0.204441) -- (1.635255,0.186006) -- (1.618034,0.193048) -- (1.607391,0.174613) -- (1.618034,0.156179) -- (1.596748,0.156179) -- (1.594235,0.174613) -- (1.572949,0.174613) -- (1.583592,0.156179) -- (1.572949,0.137745) -- (1.555728,0.144786) -- (1.545085,0.126351) -- (1.566371,0.126351) -- (1.568884,0.107917) -- (1.590170,0.107917) -- (1.600813,0.126351) -- (1.611456,0.107917) -- (1.596748,0.096524) -- (1.607391,0.078089) -- (1.628677,0.078089) -- (1.618034,0.059655) -- (1.600813,0.066696) -- (1.590170,0.048262) -- (1.611456,0.048262) -- (1.622099,0.029828) -- (1.607391,0.018434) -- (1.618034,-0.000000) -- (1.628677,0.018434) -- (1.645898,0.011393) -- (1.656541,0.029828) -- (1.645898,0.048262) -- (1.667184,0.048262) -- (1.669697,0.029828) -- (1.690983,0.029828) -- (1.680340,0.048262) -- (1.690983,0.066696) -- (1.708204,0.059655) -- (1.718847,0.078089) -- (1.697561,0.078089) -- (1.686918,0.096524) -- (1.701626,0.107917) -- (1.690983,0.126351) -- (1.712269,0.126351) -- (1.714782,0.107917) -- (1.736068,0.107917) -- (1.746711,0.126351) -- (1.757354,0.107917) -- (1.742646,0.096524) -- (1.753289,0.078089) -- (1.763932,0.096524) -- (1.785218,0.096524) -- (1.787731,0.078089) -- (1.809017,0.078089) -- (1.798374,0.096524) -- (1.813082,0.107917) -- (1.802439,0.126351) -- (1.781153,0.126351) -- (1.791796,0.144786) -- (1.809017,0.137745) -- (1.819660,0.156179) -- (1.809017,0.174613) -- (1.830303,0.174613) -- (1.832816,0.156179) -- (1.854102,0.156179) -- (1.843459,0.174613) -- (1.854102,0.193048) -- (1.871323,0.186006) -- (1.881966,0.204441) -- (1.860680,0.204441) -- (1.858167,0.222875) -- (1.836881,0.222875) -- (1.826238,0.204441) -- (1.815595,0.222875) -- (1.830303,0.234268) -- (1.819660,0.252703) -- (1.798374,0.252703) -- (1.809017,0.271137) -- (1.826238,0.264096) -- (1.836881,0.282530) -- (1.815595,0.282530) -- (1.804952,0.300965) -- (1.819660,0.312358) -- (1.809017,0.330792) -- (1.830303,0.330792) -- (1.832816,0.312358) -- (1.854102,0.312358) -- (1.864745,0.330792) -- (1.875388,0.312358) -- (1.860680,0.300965) -- (1.871323,0.282530) -- (1.881966,0.300965) -- (1.903252,0.300965) -- (1.905765,0.282530) -- (1.927051,0.282530) -- (1.916408,0.300965) -- (1.927051,0.319399) -- (1.944272,0.312358) -- (1.954915,0.330792) -- (1.965558,0.312358) -- (1.950850,0.300965) -- (1.961493,0.282530) -- (1.982779,0.282530) -- (1.972136,0.264096) -- (1.954915,0.271137) -- (1.944272,0.252703) -- (1.965558,0.252703) -- (1.976201,0.234268) -- (1.961493,0.222875) -- (1.972136,0.204441) -- (1.982779,0.222875) -- (2.000000,0.215834) -- (2.010643,0.234268) -- (2.000000,0.252703) -- (2.021286,0.252703) -- (2.023799,0.234268) -- (2.045085,0.234268) -- (2.055728,0.252703) -- (2.066371,0.234268) -- (2.051663,0.222875) -- (2.062306,0.204441) -- (2.072949,0.222875) -- (2.094235,0.222875) -- (2.096748,0.204441) -- (2.118034,0.204441) -- (2.107391,0.222875) -- (2.122099,0.234268) -- (2.111456,0.252703) -- (2.090170,0.252703) -- (2.100813,0.271137) -- (2.118034,0.264096) -- (2.128677,0.282530) -- (2.118034,0.300965) -- (2.139320,0.300965) -- (2.141833,0.282530) -- (2.163119,0.282530) -- (2.152476,0.300965) -- (2.163119,0.319399) -- (2.180340,0.312358) -- (2.190983,0.330792) -- (2.201626,0.312358) -- (2.186918,0.300965) -- (2.197561,0.282530) -- (2.218847,0.282530) -- (2.208204,0.264096) -- (2.190983,0.271137) -- (2.180340,0.252703) -- (2.201626,0.252703) -- (2.212269,0.234268) -- (2.197561,0.222875) -- (2.208204,0.204441) -- (2.218847,0.222875) -- (2.240133,0.222875) -- (2.242646,0.204441) -- (2.263932,0.204441) -- (2.253289,0.186006) -- (2.236068,0.193048) -- (2.225425,0.174613) -- (2.236068,0.156179) -- (2.214782,0.156179) -- (2.212269,0.174613) -- (2.190983,0.174613) -- (2.201626,0.156179) -- (2.190983,0.137745) -- (2.173762,0.144786) -- (2.163119,0.126351) -- (2.184405,0.126351) -- (2.186918,0.107917) -- (2.208204,0.107917) -- (2.218847,0.126351) -- (2.229490,0.107917) -- (2.214782,0.096524) -- (2.225425,0.078089) -- (2.246711,0.078089) -- (2.236068,0.059655) -- (2.218847,0.066696) -- (2.208204,0.048262) -- (2.229490,0.048262) -- (2.240133,0.029828) -- (2.225425,0.018434) -- (2.236068,0.000000) -- (2.246711,0.018434) -- (2.263932,0.011393) -- (2.274575,0.029828) -- (2.263932,0.048262) -- (2.285218,0.048262) -- (2.287731,0.029828) -- (2.309017,0.029828) -- (2.298374,0.048262) -- (2.309017,0.066696) -- (2.326238,0.059655) -- (2.336881,0.078089) -- (2.315595,0.078089) -- (2.304952,0.096524) -- (2.319660,0.107917) -- (2.309017,0.126351) -- (2.330303,0.126351) -- (2.332816,0.107917) -- (2.354102,0.107917) -- (2.364745,0.126351) -- (2.375388,0.107917) -- (2.360680,0.096524) -- (2.371323,0.078089) -- (2.381966,0.096524) -- (2.403252,0.096524) -- (2.405765,0.078089) -- (2.427051,0.078089) -- (2.416408,0.096524) -- (2.427051,0.114958) -- (2.444272,0.107917) -- (2.454915,0.126351) -- (2.465558,0.107917) -- (2.450850,0.096524) -- (2.461493,0.078089) -- (2.482779,0.078089) -- (2.472136,0.059655) -- (2.454915,0.066696) -- (2.444272,0.048262) -- (2.465558,0.048262) -- (2.476201,0.029828) -- (2.461493,0.018434) -- (2.472136,0.000000) -- (2.482779,0.018434) -- (2.500000,0.011393) -- (2.510643,0.029828) -- (2.500000,0.048262) -- (2.521286,0.048262) -- (2.523799,0.029828) -- (2.545085,0.029828) -- (2.555728,0.048262) -- (2.566371,0.029828) -- (2.551663,0.018434) -- (2.562306,0.000000) -- (2.572949,0.018434) -- (2.594235,0.018434) -- (2.596748,-0.000000) -- (2.618034,-0.000000)
}

